Stability of Linear Flocks on a Ring Road

We discuss some stability problems when each agent of a linear flock on the line interacts with its two nearest neighbors (one on either side).

==> inputlatex.tex <==

%\usepackage[notref,notcite]{showkeys}
\usepackage[usenames]{color}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To draw commutative diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}

\textwidth=18.00 true cm \textheight=21.50 true cm
\baselineskip=18pt \voffset=-2cm \hoffset=-2.5cm
%\parskip=8pt
\parindent=6ex
%\input{pepet.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Valencian Definitions
%Uso de las definiciones valencianas%
%Theorem
%\begin{theo}\label{***}Statement of theorem \end{theo}
%\begin{prop}\label{***}Statement of theorem \end{prop}
%\begin{lem}\label{***}Statement of theorem \end{lem}
%\begin{cory}\label{***}Statement of theorem \end{cory}
%\begin{rem}\label{***}Statement of theorem \end{rem}
%when needed:
%\setcounter{figure}{0}
%\setcounter{equation}{0}
%\setcounter{theorem}{0}
%\begin{proof}  Proof \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\newtheorem {theo} {\bf Theorem} [section]
\newtheorem {prop} [theo] {\bf Proposition}
\newtheorem {cory} [theo] {\bf Corollary}
\newtheorem {lem} [theo] {\bf Lemma}
\newtheorem {defn} [theo] {\bf Definition}
\newtheorem {conj} [theo] {\bf Conjecture}
\newtheorem {exam} [theo] {\bf Example}
\newtheorem {rem} [theo] {\bf Remark}
\newcommand{\QED}{\hfill \CaixaPreta \vspace{6mm}}
\def\CaixaPreta{\vrule Depth0pt height6pt width6pt}
\newenvironment{remark}{\begin{rem}\begin{rm}}{\end{rm}
\nopagebreak\hfill$\Box$\end{rem}\par\vspace{\partopsep}}
\newenvironment{defin}{\begin{DEFCURSIVA}\begin{rm}}{\end{rm}\end{DEFCURSIVA}}
\newenvironment{proclama}[1]{\par\vspace{\topsep}\noindent{\bf #1}
\begin{em}}{\end{em}\par\vspace{\topsep}}
\newcommand{\qed}{\nopagebreak\hfill{\vrule width6pt height6pt depth0pt}}
%\newenvironment{proof}{\noindent{\bf Proof:}}{\qed\par
%\vspace{\topsep}\vspace{\partopsep}}
\newenvironment{proof}[1]{\vspace{0.4 cm}\noindent{\em #1.}}{\qed\par
\vspace{\topsep}\vspace{\partopsep}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dpy}{\displaystyle}
%eqn array with numbered lines:
%use & to align, \\ for new line, \\[0.4cm] for new line and add'l vert. space.
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
%eqn array no number:
\newcommand{\benn}{\begin{eqnarray*}}
\newcommand{\eenn}{\end{eqnarray*}}
%single eqn numbered:
\newcommand{\bse}{\begin{equation}}
\newcommand{\ese}{\end{equation}}
%single eqn no number:
\newcommand{\bsenn}{\begin{displaymath}}
\newcommand{\esenn}{\end{displaymath}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Some Functions (math style)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\logand}{\;\;{\rm and }\;\;}
\newcommand{\for}{\;\;{\rm for }\;\;}
\newcommand{\logor}{\;\;{\rm or }\;\;}
\newcommand{\logif}{\;\;{\rm if }\;\;}
\newcommand{\logelse}{\;\;{\rm else }\;\;}
\newcommand{\then}{\;\;{\rm then }\;\;}
\newcommand{\where}{\;\;{\rm where }\;\;}
\newcommand{\with}{\;\;{\rm with }\;\;}
\newcommand{\such}{\;\;{\rm such\; that }\;\;}
\newcommand{\limcap}{\;{\rm d }\,}
\newcommand{\Tr}{\;{\rm Tr }\,}
\newcommand{\Hd}{\;{\rm Hd }\,}
\newcommand{\atanh}{\;{\rm arctanh }\,}
\newcommand{\Hdim}{\;{\rm Hdim }\,}
\newcommand{\Hlim}{\;{\rm Hlim }\,}
\newcommand{\card}{\;{\rm card }\,}
\newcommand{\Id}{\,{\rm Id}\,}
%\newcommand{\mod}{\bmod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Other
%%('re' is added because \O and \S are existing commands)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{\mbox{I${\!\!\!}$C}}
\renewcommand{\O}{\mbox{I${\!\!\!}$O}}
\renewcommand{\H}{\mbox{I${\!\!\!}$H}}
\newcommand{\Q}{\mbox{I${\!\!\!}$Q}}
\newcommand{\G}{\mbox{I${\!\!\!}$G}}
\newcommand{\T}{\mbox{T${\!\!\!}$T}}
\newcommand{\N}{\mbox{I${\!}$N}}
\newcommand{\R}{\mbox{I${\!}$R}}
\newcommand{\D}{\mbox{I${\!}$D}}
\newcommand{\Z}{\mbox{Z${\!\!}$Z}}
\renewcommand{\S}{\mbox{S${\!\!\!\!}$S}}
\newcommand{\CaixaBranca}{$\Box$}
\newcommand{\creu}{{\rule[-0.1mm]{2mm}{0.2mm}\rule{0.1mm}{2.5mm}}}
\newcommand{\ca}{\c ca }
\newcommand{\co}{\c co }
\newcommand{\mv}{mente, }
\newcommand{\caop}{\c c\~ao. }
\newcommand{\caov}{\c c\~ao, }
\newcommand{\coesp}{\c c\~oes. }
\newcommand{\coesv}{\c c\~oes, }
\newcommand{\cao}{\c c\~ao }
\newcommand{\CAO}{\c C\~AO }
\newcommand{\coes}{\c c\~oes }
\newcommand{\COES}{\c C\~OES }
\newcommand{\sao}{s\~ao }
\newcommand{\SAO}{S\~AO }
\newcommand{\m}{mente }
\newcommand{\ii}{\'{\i}}

